Nature vs. Nurture: The Role of Environmental Resources in Evolutionary Deep Intelligence

Evolutionary deep intelligence synthesizes highly efficient deep neural networks architectures over successive generations. Inspired by the nature versus nurture debate, we propose a study to examine the role of external factors on the network synthesis process by varying the availability of simulated environmental resources. Experimental results were obtained for networks synthesized via asexual evolutionary synthesis (1-parent) and sexual evolutionary synthesis (2-parent, 3-parent, and 5-parent) using a 10% subset of the MNIST dataset. Results show that a lower environmental factor model resulted in a more gradual loss in performance accuracy and decrease in storage size. This potentially allows significantly reduced storage size with minimal to no drop in performance accuracy, and the best networks were synthesized using the lowest environmental factor models.

==> Background.tex <==
Following the seminal evolutionary deep intelligence paper~\cite{Shafiee2016}, Shafiee~\textit{et al.}~\cite{Shafiee2016_2} further proposed a detailed extension of the original approach via synaptic cluster-driven genetic encoding. This work further examined the genetic encoding scheme used to mimic heredity in neural networks across generations, and introduced a multi-factor synapse probability model that encodes the synaptic probability as a product of the synthesis probability of a cluster of synapses and the synthesis probability of a particular synapse within the cluster. Shafiee~\textit{et al.}'s new genetic encoding scheme produced significantly more efficient network architectures specifically tailored for GPU-accelerated applications while maintaining state-of-the-art performance accuracy.

Shafiee~\textit{et al.}~\cite{Shafiee2017} further demonstrated the efficacy of the synaptic cluster-driven genetic encoding scheme via comprehensive experimental results using four well-known deep neural networks (LeNet-5~\cite{LeCun1998_LeNet}, AlexNet~\cite{Krizhevsky2012}, ResNet-65~\cite{He2016}, and DetectNet which is derived from GoogleNet~\cite{Szegedy2015}) on both object recognition and object detection tasks. The resulting synthesized offspring networks had significantly more efficient network architectures that achieved state-of-the-art performance, in addition to being well-tailored to embedded parallel computation devices.

Shafiee~\textit{et al.}~\cite{Shafiee2017_Restrictions} also investigated the imposition of a synaptic precision constraint during the evolutionary synthesis of network architectures. Enforcing a half-precision (16-bit) synaptic constraint at each generation and training the synthesized networks at full precision (32-bit), the resulting synthesized networks had significantly fewer synapses and reduced precision requirements while maintaining performance accuracy.

Most recently, Shafiee~\textit{et al.}~\cite{Shafiee2017_Transgenerational} introduced the concept of trans-generational genetic transmission of environmental information within the evolutionary deep intelligence approach. Favouring the synthesis of increasingly efficient neural network architectures over successive generations, Shafiee~\textit{et al.} imposes intra-generational traumatic environmental stresses to weaken the strengths of a subset of synapses during training. The transmission of environmental information from generation to generation resulted in deep neural networks with a notable increase in architectural efficiency and comparable performance accuracy relative to networks synthesized via the original cluster-driven evolutionary deep intelligence method~\cite{Shafiee2016_2}.

The previous work in evolutionary deep intelligence, however, formulated the evolutionary synthesis process based on asexual reproduction (i.e., new neural networks are synthesized using a single parent network). Chung~\textit{et al.}~\cite{Chung2017_Mating} extended the asexual evolutionary sythensis approach via the incorporation of a second parent network, showing that networks synthesized via sexual evolutionary synthesis had approximately double the architectural efficiency of networks synthesized using asexual evolutionary synthesis with comparable performance accuracy. Chung~\textit{et al.}~\cite{Chung2017_Polyploidism} further investigated the effects of $m$-parent evolutionary synthesis (for $m = 1, 2, 3, 5$) in varying population sizes of three, five, and eight networks per generation, demonstrating that increasing the number of parent networks resulted in synthesizing networks with improved architectural efficiency with only a $2 - 3\%$ drop in performance accuracy.

